Predicting Sight and Sound for Audio-Visual Perception, World Modeling and Intuitive Physics

Sight and sound provide complementary supervision on a shared time axis. Yet, audio-visual (AV) self-supervised methods commonly encode the two streams separately and align them only per clip, and few benchmarks require integrating them; we address both gaps. We introduce JEP-AV, a joint-embedding predictive architecture whose single transformer encodes video, audio, or both over a shared time axis. It predicts a teacher's assignments to learned prototypes (ProtoLoss) within and across modalities, using token-level and 500 ms chunk-level targets. Building on JEP-AV, we explore world modeling over its representation space: AVJ-WM, an autoregressive world model with modules designed for its features, predicts future AV states and plans through lightweight action adapters, and we compare it with diffusion world models (CDiT) trained on the same features. To evaluate cross-modal integration, we introduce two benchmarks: IntPhys-X, whose intuitive physics tasks can only be solved by combining sight and sound, from matching the two streams to reasoning over sound-action associations in context, and AVNav-Bench, in which the world model itself plans toward image or sound goals. JEP-AV sets the state of the art among frozen self-supervised encoders on audio and AV classification and on sound-prompted segmentation. On AVNav-Bench, AVJ-WM reaches the highest success on distant and sound goals, scoring 39.6% and 19.1% vs. at most 26.9% and 5.1% for diffusion world models. On IntPhys-X, JEP-AV averages 65.5% on the no-context scenarios, ahead of all representation models and on par with Gemini-4 Argon (65.3%). Humans reach 84-99%, whereas the best model in each scenario trails them by over 20 points on average. Cross-modal physical understanding remains an open challenge.

==> figures/03_audio_visual_results/01_DenseAVFeats/av_tsne_semantic_v3/av_tsne_semantic_v3_overlay.tex <==
\definecolor{avtsnwC0}{HTML}{660C01}%
\definecolor{avtsnwC1}{HTML}{B75463}%
\definecolor{avtsnwC2}{HTML}{FE8E99}%
\definecolor{avtsnwC3}{HTML}{00295D}%
\definecolor{avtsnwC4}{HTML}{2770A6}%
\definecolor{avtsnwC5}{HTML}{62ABF3}%
\definecolor{avtsnwC6}{HTML}{145439}%
\definecolor{avtsnwC7}{HTML}{0CBA62}%
\definecolor{avtsnwC8}{HTML}{9CE694}%
\definecolor{avtsnwC9}{HTML}{815702}%
\definecolor{avtsnwC10}{HTML}{E76E00}%
\definecolor{avtsnwC11}{HTML}{FABA2F}%
\definecolor{avtsnwC12}{HTML}{61359F}%
\definecolor{avtsnwC13}{HTML}{8E71FD}%
\definecolor{avtsnwC14}{HTML}{CCC5FA}%
\def\avtsnwAspectBalanced{1.11901}%
\def\avtsnwAspectPlain{1.05584}%
\def\avtsnwOverlayBalanced{%
  \avtsnwLabel{0.6503}{0.5095}{avtsnwC5}{motorboat}%
  \avtsnwLabel{0.7404}{0.4245}{avtsnwC9}{surf}%
  \avtsnwLabel{0.4817}{0.9283}{avtsnwC1}{rooster}%
  \avtsnwLabel{0.5756}{0.8238}{avtsnwC2}{cow}%
  \avtsnwLabel{0.2860}{0.1155}{avtsnwC6}{piano}%
  \avtsnwLabel{0.1456}{0.2168}{avtsnwC8}{drum kit}%
  \avtsnwLabel{0.7294}{0.3249}{avtsnwC10}{waterfall}%
  \avtsnwLabel{0.6860}{0.6168}{avtsnwC11}{fire}%
  \avtsnwLabel{0.2283}{0.8033}{avtsnwC0}{dog}%
  \avtsnwLabel{0.8862}{0.7220}{avtsnwC3}{train}%
  \avtsnwLabel{0.8437}{0.5309}{avtsnwC4}{airplane}%
  \avtsnwLabel{0.4533}{0.0733}{avtsnwC7}{bagpipes}%
  \avtsnwLabel{0.4377}{0.6343}{avtsnwC12}{vacuum cleaner}%
  \avtsnwLabel{0.1685}{0.4714}{avtsnwC13}{toilet flush}%
  \avtsnwLabel{0.1225}{0.5407}{avtsnwC14}{frying}%
}
\def\avtsnwOverlayPlain{%
  \avtsnwLabel{0.5936}{0.4422}{avtsnwC5}{motorboat}%
  \avtsnwLabel{0.4407}{0.1877}{avtsnwC6}{piano}%
  \avtsnwLabel{0.7321}{0.3870}{avtsnwC9}{surf}%
  \avtsnwLabel{0.6540}{0.3055}{avtsnwC10}{waterfall}%
  \avtsnwLabel{0.3991}{0.9364}{avtsnwC1}{rooster}%
  \avtsnwLabel{0.5782}{0.7930}{avtsnwC2}{cow}%
  \avtsnwLabel{0.6026}{0.0903}{avtsnwC7}{bagpipes}%
  \avtsnwLabel{0.3007}{0.2040}{avtsnwC8}{drum kit}%
  \avtsnwLabel{0.1541}{0.4550}{avtsnwC13}{toilet flush}%
  \avtsnwLabel{0.0501}{0.5186}{avtsnwC14}{frying}%
  \avtsnwLabel{0.3656}{0.7978}{avtsnwC0}{dog}%
  \avtsnwLabel{0.9651}{0.6908}{avtsnwC3}{train}%
  \avtsnwLabel{0.8718}{0.5433}{avtsnwC4}{airplane}%
  \avtsnwLabel{0.6488}{0.6124}{avtsnwC11}{fire}%
  \avtsnwLabel{0.3871}{0.5666}{avtsnwC12}{vacuum cleaner}%
}


==> figures/06_intuitive_physics/intphysx_structure/intphysx_structure_helpers.tex <==
\tikzset{line join=round,
  isx/card/.style={fill=avGrid!45, draw=none, rounded corners=3pt},
  isx/title/.style={font=\footnotesize\bfseries, text=avInk, inner sep=0pt, anchor=base west},
  isx/fam/.style={font=\scriptsize, text=avInk2, inner sep=0pt, anchor=north west, align=left},
  isx/lbl/.style={font=\scriptsize, text=avInk2, inner sep=0.5pt},
  isx/onbg/.style={fill=avGrid!45, inner sep=0.6pt},  %
  isx/num/.style={circle, fill=avInk2, text=white, font=\scriptsize\bfseries, inner sep=0pt,
    minimum size=3.3mm},
  isx/ab/.style={rounded corners=0.5mm, fill=#1, text=white, font=\scriptsize\bfseries,
    inner sep=0pt, minimum size=2.9mm},
  isx/arr/.style={-{Stealth[length=1.15mm,width=1mm]}, line width=0.45pt, color=avInk2},
  isx/model/.style={draw=avInk2, fill=white, line width=0.5pt, rounded corners=2pt,
    font=\scriptsize, text=avInk, align=center, inner sep=1pt, minimum height=8mm,
    minimum width=12mm},
  isx/decide/.style={fill=white, draw=avAxis, line width=0.45pt, rounded corners=2pt,
    minimum width=25mm, minimum height=10.5mm, font=\scriptsize, text=avInk,
    align=center, inner sep=1pt},
  isx/tt/.style={fill=white, draw=avInk2, line width=0.45pt, rounded corners=2pt,
    font=\ttfamily\scriptsize, text=avInk, inner xsep=1.6pt, inner ysep=1.4pt},
  isx/guide/.style={draw=avMuted, line width=0.4pt, dash pattern=on 1pt off 0.9pt},
  isx/axis/.style={draw=avAxis, line width=0.5pt},
  isx/hatch/.style={pattern=north east lines, pattern color=avMuted},}
\def\isxWave#1#2#3#4#5#6#7#8#9{%
  \foreach \isxI in {0,...,#6} {
    \pgfmathsetmacro{\isxX}{#1+\isxI*#3/#6}
    \pgfmathsetmacro{\isxJ}{\isxI-#9}
    \pgfmathsetmacro{\isxT}{#1+\isxJ*#3/#6}
    \pgfmathsetmacro{\isxUa}{\isxT-#7}
    \pgfmathsetmacro{\isxUb}{\isxT-#8}
    \pgfmathsetmacro{\isxEnv}{min(1, 0.13
        + (\isxUa>=0)*exp(-max(\isxUa,0)/2.2)*min(1,0.45+\isxUa/0.6)
        + 0.85*(\isxUb>=0)*exp(-max(\isxUb,0)/2.2)*min(1,0.45+\isxUb/0.6))}
    \pgfmathsetmacro{\isxAmp}{#4*\isxEnv*(0.35+0.65*abs(sin(\isxJ*67+11)*cos(\isxJ*29+23)))}
    \draw[#5, line width=0.42pt] (\isxX,{#2-\isxAmp}) -- (\isxX,{#2+\isxAmp});
  }}
\def\isxFrame#1#2#3#4#5#6#7{%
  \begin{scope}
    \clip[rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);
    \fill[cVideo!9] (#1,#2) rectangle ++(#3,#4);
    \fill[cVideo!38] (#1,#2) rectangle ++(#3,{0.2*#4});
  \end{scope}
  \pgfmathsetmacro{\isxR}{0.125*#4}
  \pgfmathsetmacro{\isxBx}{#1+#5*#3}
  \pgfmathsetmacro{\isxGy}{#2+0.2*#4}
  \pgfmathsetmacro{\isxBy}{\isxGy+\isxR+#6*(0.8*#4-2.6*\isxR)}
  \fill[cVideo!75!black] (\isxBx,\isxBy) circle (\isxR);
  \ifnum#7=1
    \draw[cVideo!75!black, line width=0.4pt]
      ({\isxBx-1.45*\isxR},{\isxGy+0.25*\isxR}) -- ++({-0.9*\isxR},{0.45*\isxR})
      ({\isxBx-1.3*\isxR},{\isxGy+1.05*\isxR}) -- ++({-0.75*\isxR},{0.75*\isxR})
      ({\isxBx+1.45*\isxR},{\isxGy+0.25*\isxR}) -- ++({0.9*\isxR},{0.45*\isxR})
      ({\isxBx+1.3*\isxR},{\isxGy+1.05*\isxR}) -- ++({0.75*\isxR},{0.75*\isxR});
  \fi
  \draw[cVideo!75!black, line width=0.4pt, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);}
\def\isxTS{0.6}\def\isxTW{0.75}
\def\isxTone#1#2#3{\draw[cAudio!75!black, line width=0.9pt] ({#1-\isxTW},{#2+0.25+\isxTS*#3}) -- ({#1+\isxTW},{#2+0.25+\isxTS*#3});}
\def\isxTH{3.0}
\def\isxTrack#1#2#3{\fill[cAudio!10] (#1,#3) rectangle (#2,#3+\isxTH);
  \draw[cAudio!60!black, line width=0.4pt] (#1,#3) rectangle (#2,#3+\isxTH);}
\def\isxNoVideo#1#2#3#4{\fill[white] (#1,#3) rectangle (#2,#3+#4);
  \fill[isx/hatch] (#1,#3) rectangle (#2,#3+#4);
  \draw[avMuted, line width=0.4pt] (#1,#3) rectangle (#2,#3+#4);
  \node[isx/lbl, isx/onbg, font=\scriptsize\itshape] at ({(#1+#2)/2},{#3+#4/2}) {no video};}
\def\isxSimon#1#2#3#4#5{%
  \fill[avInk!88, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);
  \pgfmathsetmacro{\isxPw}{0.32*#3}\pgfmathsetmacro{\isxPh}{0.34*#4}
  \foreach \isxP/\isxC/\isxDx/\isxDy in {1/avOrange/0.14/0.56, 2/avYellow/0.54/0.56, 3/avViolet/0.14/0.10, 4/avMagenta/0.54/0.10} {
    \pgfmathtruncatemacro{\isxOn}{(\isxP==#5) ? 1 : 0}
    \ifnum\isxOn=1 \def\isxF{\isxC}\else\def\isxF{\isxC!25!avMuted!70!avInk}\fi
    \fill[\isxF, rounded corners=0.25mm] ({#1+\isxDx*#3},{#2+\isxDy*#4}) rectangle ++(\isxPw,\isxPh);}}
\def\isxBoard#1#2#3#4#5#6{%
  \fill[cVideo!9, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);
  \foreach \isxJ in {1,...,5} {\draw[cVideo!30, line width=0.3pt] ({#1+\isxJ*#3/6},#2) -- ++(0,#4);}
  \draw[cVideo!30, line width=0.3pt] (#1,{#2+#4/2}) -- ++(#3,0);
  \fill[cVideo!75!black] ({#1+(#5+0.5)*#3/6},{#2+0.75*#4}) circle ({0.17*#4});
  \fill[avOrange!85!black] ({#1+(#6+0.5)*#3/6-0.19*#4},{#2+0.08*#4}) -- ++({0.38*#4},0) -- ++({-0.19*#4},{0.34*#4}) -- cycle;
  \draw[cVideo!75!black, line width=0.4pt, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);}
\def\isxCups#1#2#3#4#5#6#7{%
  \fill[cVideo!9, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);
  \foreach \isxJ in {1,2,3} {
    \pgfmathsetmacro{\isxCx}{#1+(\isxJ-0.5)*#3/3}
    \pgfmathtruncatemacro{\isxUp}{(\isxJ==#5) ? 1 : 0}
    \pgfmathsetmacro{\isxLift}{\isxUp*0.28*#4}
    \ifnum\isxUp=1 \fill[avOrange!85!black] (\isxCx,{#2+0.2*#4}) circle ({0.09*#4}); \fi
    \fill[cVideo!70!black] ({\isxCx-0.12*#3},{#2+0.12*#4+\isxLift}) -- ({\isxCx+0.12*#3},{#2+0.12*#4+\isxLift})
      -- ({\isxCx+0.08*#3},{#2+0.55*#4+\isxLift}) -- ({\isxCx-0.08*#3},{#2+0.55*#4+\isxLift}) -- cycle;}
  \ifnum#6>0
    \draw[{Stealth[length=0.7mm,width=0.6mm]}-{Stealth[length=0.7mm,width=0.6mm]}, avInk2, line width=0.4pt]
      ({#1+(#6-0.5)*#3/3},{#2+0.66*#4}) .. controls ({#1+(#6-0.5)*#3/3},{#2+0.95*#4}) and ({#1+(#7-0.5)*#3/3},{#2+0.95*#4}) .. ({#1+(#7-0.5)*#3/3},{#2+0.66*#4});
  \fi
  \draw[cVideo!75!black, line width=0.4pt, rounded corners=0.45mm] (#1,#2) rectangle ++(#3,#4);}
\def\isxChip#1#2#3#4#5#6{%
  \fill[avGrid!45, rounded corners=2pt] (#1,#2) rectangle ++(#3,#4);
  \node[isx/lbl, anchor=base west, inner sep=0pt, font=\scriptsize, text=avInk] at ({#1+1.4},{#2+#4-2.75}) {#5};
  \node[isx/lbl, anchor=base west, inner sep=0pt, font=\scriptsize] at ({#1+1.4},{#2+#4-5.45}) {#6};}
\def\isxCorrect{\textcolor{cAudio!80!black}{\ding{51}}}
\def\isxWrong{\textcolor{cLoss}{\ding{55}}}

